Dashlet: Taming Swipe Uncertainty for Robust Short Video Streaming

Short video streaming applications have recently gained substantial traction, but the non-linear video presentation they afford swiping users fundamentally changes the problem of maximizing user quality of experience in the face of the vagaries of network throughput and user swipe timing. This paper describes the design and implementation of Dashlet, a system tailored for high quality of experience in short video streaming applications. With the insights we glean from an in-the-wild TikTok performance study and a user study focused on swipe patterns, Dashlet proposes a novel out-of-order video chunk pre-buffering mechanism that leverages a simple, non machine learning-based model of users' swipe statistics to determine the pre-buffering order and bitrate. The net result is a system that achieves 77-99% of an oracle system's QoE and outperforms TikTok by 43.9-45.1x, while also reducing by 30% the number of bytes wasted on downloaded video that is never watched.

==> Comparison.tex <==
\section{Short vs Traditional video streaming}
\label{s:comparison}

\rn{this section doesn't really compare/contrast with traditional streaming. I wonder if there is really anything that is different in the modeling? it seems like it is the exact same modeling as with traditional streaming, except that only stuff that is actually viewed is considered in the QoE? if so, then I think you can just say that succinctly and just start with Section 3, and present an overview of the short streaming environment as 3.1 to help characterize the study/results.}

\rn{perhaps would be good to mention how the app knows what the 'next' videos are?}
\subsection{System Architecture of Short Video APP}
Figure~\ref{fig:sys_arch} depicts the system architecture of short video app.
The video player fetches short videos from the video buffer for rendering 
and switches to the next video if the user swipes. 
The video buffer stores the chunks of multiple videos, 
preventing \rn{prevent feels too strong} the rebuffering event from happening when the user swipes.
The ABR algorithm fills the video buffer by sending an HTTPS request to the CDN server to 
request a certain video chunk \rn{from a specific video}.
To maximize the QoE of the user, before sending the request,
the ABR algorithm makes three decisions according to the network capacity and user swipes: 
which video and which chunk inside the selected video we should download,
and what quality of the video we should request. \rn{is this written based off of a certain algorithm? e.g., are swipes incorporated in that decision?}
\begin{figure}[t]
    \centering
        \includegraphics[width=\linewidth]{pix/Mea_arch.pdf}
        \caption{General system architecture of short video applications.}
    \label{fig:sys_arch}
\end{figure}




\subsection{Short video streaming model}
\label{ss:problem-model}
With the key difference between short and traditional video streaming in mind \rn{what are the key differences? perhaps rephrase that this is for context for the rest of the paper?}, we introduce a formal modeling about short video streaming problem. 
We model short video streams as a sequence of videos, $S={s_1, \ldots, s_k}$ that is watched by the user. Each video is encoded into $c_i$ different chunks represented by ${s_{i1}, \ldots, s_{ic_i}}$. For each chunk $s_{ij}$, the ABR algorithm can choose whether to download it or not and also the corresponding bitrate $b_{ij}$ and buffer order. The goal of the algorithm is to maximize the quality of experience when a user finishes watching the sequence of video $S={s_1, \ldots, s_k}$.


\paragraph{Quality of Experience (QoE).} We follow the traditional QoE definition of previous papers~\cite{todo}. The QoE includes the bitrate rewards, which gives high rewards for serving user higher bitrate video, the rebuffering penalty which penalize the rebuffering, and the smoothness penalty, which penalize the bitrate switching. 
\begin{equation}
    QoE = Reward_{bitrate} - \mu \cdot Penalty_{rebuffer} - \eta \cdot Penalty_{smooth}
\end{equation}
where $\mu$ and $\eta$ are the rebuffering penalty weight and smoothness penalty weight correspondingly. 

\paragraph{Bitrate reward.} In short video streaming, not all chunks in a video will \rn{must, not will} be watched by a user. When computing the reward, only the part of video that is watched should count. Suppose for video $s_i$, the first $w_i$ chunks are watched and the user spends $t_{i1}, \ldots, t_{iw_i}$ seconds on the corresponding chunks. 
Then the bitrate reward can be defined as:
    \begin{equation} Reward_{bitrate} =  \sum_{i=1}^{k}\sum_{j=1}^{w_i} b_{ij} t_{ij}
    \label{eq:reward-define}
    \end{equation}
The short video application does not allow users seek the playback within a short video. Therefore, $t_{ij}$ equals to the chunk duration for all the chunks except the last watched chunk for every video. 

\paragraph{Rebuffer penalty:} Rebuffering happens when the player needs to play a video chunk, but it is not fully downloaded yet.Suppose the time that chunk $s_{ij}$ should start to play is $p_{ij}$ and the time that chunk $s_ij$ is fully downloaded is $k_{ij}$. The rebuffering time $z_{ij}$ is $\text{max}(k_{ij}-p_{ij}, 0)$. Then the total rebuffering penalty is:
\begin{equation} 
    Penalty_{rebuffer} = \sum_{i=1}^{k}\sum_{j=1}^{w_i} \text{max}(k_{ij}-p_{ij}, 0)
    \label{eq:rebuffer-define}
\end{equation}
For a chunk $s_{ij}$, $p_{ij}$ equals to the summation of both chunk playing time $t_{ij}$ and rebuffering time $z_{ij}$ for all the chunks that are played before it. 

\paragraph{Smooth penalty:} The video quality variation within a short video will decrease the quality of experience, whereas the video quality difference among different short videos will not harm the QoE. Therefore, we define the smooth penalty as: 
    \begin{equation} 
    Penalty_{smooth} =  \sum_{i=1}^{k}\sum_{j=2}^{w_i} |b_{ij}-b_{ij-1}|
    \label{eq:smooth-define}
    \end{equation}

==> Discussion.tex <==

\section{Discussion}
\label{s:discussion}


==> Imp.tex <==
\section{Implementation}
\label{s:impl}



==> design-iterative.tex <==
\subsubsection{Iterative search}
\label{s:design:control:iterative}
In above multi-channel cases, there is no analytic solution to the optimization problem in Eq.~\ref{eqn:opt_prob}. Given a large array size and the number of possible per-element phase choices for \systemname, exhaustively searching for the optimal $\Theta$ that maximizes the objective function is too complex computationally. For example, a 4-bit phase shifter, used in \systemname, provides $2^4=16$ possible phase shifts per element and results in $16^M$ possible phase combinations for an $M$-element \systemname\ array! We therefore identify heuristics to prune the search space.

\parahead{Basic version.}
We adopt a multi-round iterative algorithm to prune the search space. 
% We adopt a multi-round iterative algorithm to search for the optimal phase combination $\Theta$. 
In each round, we sequentially align all element channels with the environmental channel. Specifically, in round one, we first align the channel $h_{p_1}$ with $h_{env}$ by searching through all possible phase settings of the first element that maximizes $F$, fixing the phases of the rest of the array.  Once we find the result, $\theta^\prime_1$, we then align the element channel $h_{p_2}$ with the intermediate combined channel $e^{j\theta^\prime_1}h_{p_1}+h_{env}$, again fixing the phases elsewhere in the array. We repeat the process for all \systemname\ elements until we obtain a vector 
$\Theta^\prime= [\theta^\prime_1, \theta^\prime_2, \dots, \theta^\prime_M]$, when this round completes.
With $\Theta^\prime$ applied to the \systemname{} elements,
the combined channel becomes
$h_{comb}\left(\Theta'\right)$:
%\begin{equation}
    % h_{comb} =\sum^M_{i=1} e^{j\Theta^\prime_i}\cdot h^1_{p(0)} + h_{env}
    %h^\prime_{comb} = e^{j\Theta^\prime}\cdot \mathbf{H_p} + h_{env}
%\end{equation}
While $F(h_{comb}(\Theta^\prime))$ usually improves over $F(h_{env})$, the improvement is not guaranteed to be optimal.
Therefore, multiple rounds of the alignment may be 
needed. These rounds proceed in much the same way as the first round, except that in subsequent rounds of alignment, when we align \systemname\ element $k$, we leave the phase of all the other elements $\Theta^{(k)} = \left[\theta_1, \ldots, \theta_{k-1}, \theta_{k+1}, \ldots, \theta_M\right]$ constant so we align element $k$ with the combined channel, $h_{comb}(\Theta^{(k)})$. We iterate until there is barely an additional 
improvement (\ie, below a threshold) in $F$ from a new 
round. The algorithm typically converges in two to three
rounds in our experiments.


By tuning one element phase at a time, the iterative algorithm already reduces the search complexity dramatically from exponential to linear: $16M$ phase settings are checked instead of $16^M$ in each round. Strictly speaking this finds the local optimal result, but we find empirically that the local optimal is typically very close to the global optimal (Figure~\ref{fig:Eval_Gap2OPT}).



\parahead{Prioritizing ``influential'' elements.}
%
Still, the execution time of our search algorithm
% a search time complexity that is linear in the \systemname\ array size 
may exceed the channel coherence time, especially when given a large \systemname\ array. Therefore, we further refine the basic iterative search as follows.

Recall that the number of \textit{dominant multipath components} in a typical indoor environment is limited to a small number~\cite{czink2004number,kotaru2015spotfi}. This suggests that the number of \textit{influential elements} in the whole \systemname\ array is also limited. Therefore, we can speed up the search and reap most of the benefit by prioritizing these influential elements.
We assign a priority level, initialized to 0, to each \systemname\ element to indicate the order of search. In each round of iteration, the elements will be reconfigured to the optimal phases in the order of their priority levels. After an element is configured, its priority level is increased by its contribution to the overall channel improvement weighted by a random probability uniformly distributed between 0 and 1. The element with the highest contribution tends to get a large increment of its priority level and will likely be tuned again sooner in the next round.

The advantages of the prioritized search algorithm are two-fold. First, the priority level ensures the element that contributes most to the channel is configured first, within the channel coherence time, and thus adapting \systemname\ quickly to changing environmental channels, which helps to mitigate the effect of mobility. Second, the algorithm does not exclude less influential elements and can still converge to the result calculated by the basic iterative algorithm.


%\parahead{Prioritizing significant phases.}


==> design-multi-obj.tex <==
\subsection{Multi\hyp{}objective control}
\label{s:design:control:multi-objective}

\parahead{Wideband single-antenna links.}
Wireless links typically operate over a wide frequency band and therefore experience frequency selective fading. This means that even a single-antenna link is comprised of a set of distinct channels, corresponding to different frequency components (subcarriers). In other words, the environmental channel $\mathbf{h_{env}}$ and the combined channel $\mathbf{h_{comb}}$ become vectors, whose length is the number of subcarriers. We can still resort to Eq.~\ref{eqn:prog_chan}, but now each element channel $\mathbf{h_{p_i}}$ is also a vector. Since our phase shifters operate over the entire frequency band without regard for subcarriers, and so the same phase shift will be applied to all subcarriers. Clearly we cannot optimize for different channels simultaneously with one phase shift configuration. Therefore, while we can still define an objective function $F$ over all subcarriers, for example, the total Shannon capacity (\ie, summing the per-subcarrier Shannon capacity), $F$ can no longer be maximized analytically.
% Fortunately, our search algorithm is generic as long as the appropriate channel expression and objective function are plugged into the optimization problem (Eq.~\ref{eqn:opt_prob}). However, the gap from the output of our algorithm to the optimal result may increase slightly. 

\parahead{Multi\hyp{}antenna (MIMO) links.}
\label{sec:wide_mimo}
\label{s:design:arch:mimo}
%
MIMO links, narrowband or wideband, are another form of "multi-channel" links. Therefore, following a similar approach used to handling wideband single-antenna links, we can derive the appropriate expressions for the channels (using Eq.~\ref{eqn:prog_chan}) and the objective function, then again use the same optimization problem formulation (Eq.~\ref{eqn:opt_prob}). For example, the situation for \textit{narrowband MIMO} links (though not seen in practical wireless technologies) is analogous to that of \textit{wideband single-antenna} links. The environmental channel $\mathbf{h_{env}}$ and the combined channel $\mathbf{h_{comb}}$ are now both \textit{matrices}, whose dimensions are determined by the number of antennas at the wireless sender and receiver respectively. Eq.~\ref{eqn:prog_chan} is still valid, but each element channel $\mathbf{h_{p_i}}$ is now also a matrix of the same dimension as that of $\mathbf{h_{env}}$ and $\mathbf{h_{comb}}$. The MIMO channel capacity is an example for the objective function.

Extending this further to \textit{wideband MIMO} links used in Wi-Fi or LTE, the environmental channel $\mathbf{h_{env}}$, the combined channel $\mathbf{h_{comb}}$, and each element channel $\mathbf{h_{p_i}}$ are all matrices of the form $N_{rx} \times N_{tx} \times N_{subcarriers}$, where $N_{rx}$, $N_{tx}$, and $N_{subcarriers}$ are the numbers of the receiver antennas, the sender antennas, and the subcarriers respectively.


\parahead{Multiple links.}
\label{s:design:arch:multinet}
%
Only single-link (SISO or MIMO) scenarios have been considered so far. Next, we extend \systemname\ to multi-link scenarios and discuss two representative cases: (i) a single cell with multiple clients associated with the same access point (AP) and on the same frequency; and (ii) multiple concurrent links on different frequencies. 

In the first case, while the AP only communicates with one client at a time, \systemname\ cannot predict which client will be active and cannot configure the element array accordingly before the transmission. Therefore,  \systemname\ configures the element array to maximize the total capacity of all AP-client links and keep the configuration until any client joins or leaves the network. In the second case, %multiple links may transmit concurrently so that 
\systemname\ must find a configuration of the element array that works for multiple links simultaneously. This can again be reduced to maximizing the total capacity. In either case, we use the total capacity expression as the objective function in our optimization problem (Eq.~\ref{eqn:opt_prob}). In addition, we adjust the objective function to consider fairness or other performance goals, \change{\ie, we maximize the aggregate capacity of all the links with the constraint that no individual link will be harmed in terms of capacity. }

% , we can again resort to the same iterative control algorithm. Similarly, 


% In either case, once we plug the total throughput expression as the objective function into our optimization problem (Eq.~\ref{eqn:opt_prob}), we can again resort to the same iterative control algorithm. Similarly, we can also adjust the objective function to consider fairness or other performance goals. 

==> design_decomp.tex <==
\subsubsection{Channel decomposition}
\label{s:design:decomp}
Our first task is to separate (decompose) the ambient environment's 
channel $h_{env}$ from the channel corresponding to the propagation
paths traversing the $i^{th}$ \systemname{} 
element.  
Suppose the $i^{th}$ \systemname{} element is configured with
phase setting $\theta_i$. We refer to the channel through 
that \systemname{} element in isolation as $e^{j\theta}h_{p_i}$.
With \systemname{} in mind, we can model the combined wireless channel 
differently than the traditional wireless channel model of 
Equation~\ref{eqn:trad_wireless} and instead write the combined 
channel in terms of the ambient environment and each 
of $M$ \systemname{} elements:
\begin{equation}
    h_{comb} = h_{env} + \sum_{i=1}^{M}e^{j\theta_i}h_{p_i}
    \label{eqn:laia_channel}
\end{equation}
We start from a simplified algorithm to decompose the channel in the 
presence of only a single 
\systemname{} element before generalizing to 
the realistic, multi\hyp{}element case.

\paragraph{Single \systemname{} element case.}
In the case of single element, the channel is comprised of the 
environment $h_{env}$, plus that element's contribution, $h_{p_1}$, supposing
the element is initially configured at $0^\circ$ phase.
We first measure the channel with the element in the $0^\circ$
state ($h_{env} + h_{p_1}$), 
then flip the element's phase to $180^\circ$ and measure the channel again
($h_{env} - h_{p_1}$).
The two resulting measured channels can be 
represented in matrix form as
\begin{equation}
\left[ \begin{array}{c}
     h_{comb}^1  \\
     h_{comb}^2 
\end{array}\right] = \left[ \begin{array}{cc}
     1  & 1 \\
     -1 & 1
\end{array}\right] \left[ \begin{array}{c}
     h_{p_1}  \\
     h_{env} 
\end{array}\right]
\label{Eq:2-probe}
\end{equation}
and the resulting linear system solved for $h_{env}$ and $h_{p_1}$. 
Once the environmental channel is known, 
we choose $\theta_1$ such that $\angle e^{j\theta_1}h_{p_1} = \angle h_{env}$,
thus phase\hyp{}aligning the environment and \systemname{} element
channels with each other.

\paragraph{Multiple \systemname{} elements.}
We now consider the realistic case where 
$M$ \systemname{} elements are present.  We form the
channels to be decomposed into an ($M+1$)\hyp{}dimensional vector comprised
of the $M$ \systemname{} elements along with the environmental channel
itself: 
\begin{equation}
    \mathbf{h} = \left[h_{p_1}, h_{p_2}, \dots , h_{p_M}, h_{env}\right]^\intercal
\end{equation}
Then $M+1$ channel measurements with different
\systemname{} element phase settings can be expressed 
as another $M+1$ dimensional vector
$\mathbf{h_{comb}}=[h_{comb}^1,h_{comb}^2,\dots,h_{comb}^{M+1}]^\intercal$, where
\begin{equation}
    \mathbf{h_{comb} = Q\cdot h}
    \label{Eq:chan_m}
\end{equation}
and $\mathbf{Q}$ is a \emph{control matrix} whose 
$M+1$ rows correspond to $M$ different phase settings of
each \systemname{} element (adjoined with 1 for the environmental
channel which we cannot change) and whose $M+1$ columns 
correspond to each of $M+1$ channel measurements.
We now decompose the channel, obtaining
$\mathbf{h}$, by 
solving the linear system of Equation~\ref{Eq:chan_m}, and that
this solution exists whenever matrix $\mathbf{Q}$ is full rank. 

\change{
We could construct a full rank control matrix by randomly configuring the \systemname{} elements for each of the $M+1$ measurements involved. But this would generate random contributions to the perceived $\mathbf{h}$, and so the intermediate combined channel $\mathbf{h_{comb}}$ would be suboptimal. Hence we instead adopt a channel decomposition strategy such that we can achieve some alignment along with each additional channel measurement, even before we construct the entire control matrix $\mathbf{Q}$.
}



%with respect to each additional measurement via the following algorithm.

\paragraph{Flip-and-align algorithm.} \systemnames{} approach
simultaneously decomposes the wireless channel and increasing
the signal to noise ratio of the channel being decomposed while the 
measurements are taking place, thus making it more practical for networks
where traffic is ongoing and present in the background of the 
measurement process. In fact, the channel measurements are piggybacked on ongoing traffic.

We use a three\hyp{}element example to illustrate the 
flip\hyp{}and\hyp{}align algorithm. 
We begin with a ``cold start'' scenario where 
all element channels and the environmental channel are unknown. 
Since all channels are unknown, we set the phase shifter of 
all \systemname{} elements to $0^\circ$ and collect the 
first channel measurement $h_{comb}^1$. We flip the phase of the 
first element, just as Figure~\ref{fig:Design_channel_probe}(a) 
shows and then collect the second channel measurement $h_{comb}^2$. 
According to Equation~\ref{Eq:2-probe}, we can now calculate the 
channel $h_{p_1}$ of the first element and the superimposed 
channel $h_{env} + h_{p_2} + h_{p_3}$, 
where $h_{p_2}$ and $h_{p_3}$ are the channels of the 
second and third elements respectively.
Next, we rotate the channel $h_{p_1}$ to align with the 
superimposed channel, as Figure~\ref{fig:Design_channel_probe}(b) 
shows. We then flip the channel of the second element, as Figure~\ref{fig:Design_channel_probe}(c) shows, and 
collect the third channel measurement $h_{comb}^3$. 
Similarly, the channel $h_{p_2}$ of the second element and 
the superimposed channel $h_{env}+h_{p_3}$ is calculated 
using three channel measurements $h_{comb}^1$, $h_{comb}^2$, and $h_{comb}^3$.
All of the estimated channels, \textit{i.e.,} $h_{p_1}$ 
and $h_{p_2}$, are then aligned with the superimposed 
channel, as shown in Figure~\ref{fig:Design_channel_probe}~(d).
We repeat until all channels are calculated and aligned,
as Figures~\ref{fig:Design_channel_probe}(e), (f) show.

The flip\hyp{}and\hyp{}align 
control matrix $\mathbf{Q}$ is thus given 
by:\footnote{$\theta_{1,1}$ is the phase rotation calculated 
to align the first element with the superimposed channel in 
the third channel measurement, as shown 
in Figure~\ref{fig:Design_channel_probe}(b); 
$\theta_{1,2}$ and $\theta_{2,1}$ are phase rotations 
calculated to align the first and second elements with 
the superimposed channel, as shown in 
Figure~\ref{fig:Design_channel_probe}~(d).}
\begin{equation}
    \mathbf{Q} = \left[ \begin{array}{cccc}
         1                    & 1                   & 1     & 1 \\
         -1                   & 1                   & 1     & 1 \\
         e^{j\theta_{1,1}}    & -1                  & 1     & 1 \\  
         e^{j\theta_{1,2}}    & e^{j\theta_{2,1}}   & -1    & 1 
    \end{array}\right] 
    \label{Eq:chan_probe_3_element}
\end{equation}
The control matrix $\mathbf{Q}$ in Eq.~\ref{Eq:chan_probe_3_element} can be extended to include an arbitrary number of \systemname\ elements.\footnote{We prove that the control matrix $\mathbf{Q}$ is full rank in the Appendix.}

When an ongoing round of channel measurements finishes, 
\systemname{} begins a new round, 
following the same flip\hyp{}and\hyp{}align algorithm with 
the only difference being the initial phase of each \systemname{} 
element.  In the new round each \systemname{} element
begins configured with its previously\hyp{}computed phase rotation,
to leverage any correlation in the wireless channel between the
two measurement rounds that will be present if both rounds complete
at time intervals close to the channel coherence time.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% According to Eq.~\ref{Eq:chan_probe_3_element}, we can calculate the channel $h_p^1$ of \systemname\ element 1 and the superimposed channel $h_p^2+h_p^3+h_e$ after we probe the channel twice and obtain $h_{comb}^1$ and $h_{comb}^2$. We then align the channel $h_p^1$ with the superimposed channel $h_p^2+h_p^3+h_e$, by rotating channel of \systemname\ element 1 with phase $e^{j\theta_{1,1}}$. We also flip the channel of \systemname\ element 2, before performing next round of channel measurement. With the third channel measurement $h_{comb}^2$, we can calculate the channel $h_p^2$. We then algin both $h_p^1$ and $h_p^2$ with the superimposed channel $h_p^3+h_e$, by rotating channel of $h_p^1$ and $h_p^2$ by $e^{j\theta_{1,2}}$ and $e^{j\theta_{2,1}}$. We repeat this process until all channels are measured and aligned.
% A randomly generated channel measurement matrix cannot work due to three reasons. First of all, random channel measurement matrix configures the \systemname\ elements randomly, which results in uncontrolled each channel measurement is actually one packet transmission. 
% As Figure~\ref{fig:Design_channel_probe}~(a) shows, the environmental channel and \systemname\ element channels adds randomly in the first place. We measure the channel of the first \systemname\ element and then align the measured channel with the superimposed channel of the rest elements and the environment, as shown in Figure~\ref{fig:Design_channel_probe}~(b). We then measure the channel of the second element and align all measured channels, \textit{i.e.,} channel element 1 and 2, with the superimposed channel, \textit{i.e.}, channel of element 3 plus environmental channel, just as Figure~\ref{fig:Design_channel_probe}~(c) shows. We repeat the process and align all \systemname\ element channels with environmental channel, as Figure~\ref{fig:Design_channel_probe}~(d) shows.

% We leverage the fact a \systemname\ element only changes the phase of a propagation path, not the environment path. Figure~\ref{fig:decomposition} demonstrates the channel decomposition process. In the figure, the green vector is the channel for environment path on IQ plan, the blue vector is the channel for a \systemname\ path on IQ plan. The decomposition process works as follow. At the first, we set the phase of phase-shifter on \systemname\ path at $0$, and get channel $H_1$, which is $H_{1} = H_{env} + H_{\systemname}$. Then we set the phase of phase-shifter on the \systemname\ path at $\pi$ and get channel $H_2$, which is $H_{2} = H_{env} + H_{\systemname} \times e^{-j\pi}$. By shifting the \systemname\ path by $\pi$, we can decompose the environment path and \systemname\ path with the following two formula, $H_{env} = (H_{1}+H_{2})/2$ and $H_{\systemname} = (H_{1}-H_{2})/2$. So we can distinguish the \systemname\ channel from the environmental channel by shifting the phase for \systemname\ path.  

% \begin{figure}[!htb]
% %\vspace{-12pt}
%   \begin{center}
%       \subfigure[]{
%       \includegraphics[width=0.22\textwidth]{pix/decomposition1.pdf}
%       \label{fig:decomposition1}}
%       %\hspace{-8pt}
%       \subfigure[]{
%       \includegraphics[width=0.22\textwidth]{pix/decomposition2.pdf}
%       \label{fig:decomposition2}}
%       % \vspace{-3pt}
%       \caption{Channel decomposition.}\label{fig:decomposition}
%   \end{center}
% % \vspace{-15pt}
% \end{figure}

% \subsubsection{Multiple \systemname\ elements}
% The channel becomes 
% Another challenge for channel decomposition is scaling up to multiple \systemname\ element. In this case, when we decompose 

% For the case when we have multiple \systemname\ elements in the system. We can first measure the channel $H_{env} + \sum_i^n H_{press_i}$. Then we can decompose $H_{press_i}$ one by one. At last, we can subtract $H_{press_i}$ from $H_{env} + \sum_i^n H_{press_i}$ to get the environmental channel $H_{env}$.

% \begin{figure*}[!htb]
% %\vspace{-12pt}
%   \begin{center}
%       \includegraphics[width=0.99\linewidth]{pix/n12.pdf}
%       \caption{Control example}
%       \label{fig:control_example}
%   \end{center}
% % \vspace{-15pt}
% \end{figure*}

% \begin{equation}
%     \left[ \begin{array}{c}
%          h_{comb}^1    \\
%          h_{comb}^2    \\
%          h_{comb}^3    \\
%          h_{comb}^4    \\
%     \end{array}\right] = \left[ \begin{array}{cccc}
%          1                    & 1                   & 1     & 1 \\
%          -1                   & 1                   & 1     & 1 \\
%          e^{j\theta_{1,1}}    & -1                  & 1     & 1 \\  
%          e^{j\theta_{1,2}}    & e^{j\theta_{2,1}}   & -1    & 1 
%     \end{array}\right] \left[ \begin{array}{c}
%          h_p^1  \\
%          h_p^2  \\
%          h_p^3  \\
%          h_e  \\
%     \end{array}\right]
%     \label{Eq:chan_probe_3_element}
% \end{equation}

==> eval_micro.tex <==
\subsection{Microbenchmarks}
\label{s:eval:micro}
\begin{figure}
%\vspace{-12pt}
  \begin{minipage}[t]{0.49\linewidth}
      \centering
      \includegraphics[width=\linewidth]{pix/scatter.pdf}
      \caption{\change{\systemname{} SNR improvement versus signal strength for six links (one point per subcarrier).}}
      \label{fig:Eval_scatter}
  \end{minipage}\hfill
  \begin{minipage}[t]{0.49\linewidth}
     \centering
     \includegraphics[width=\linewidth]{pix/Eval_array_control.pdf}
     \caption{Controllability distribution of the 36-element \systemname\ array, across 30 links.}
     \label{fig:Eval_array_control}
   \end{minipage}
\end{figure}

We conduct microbenchmarks to better understand the performance of each part of \systemname's design. The experiments to evaluate the controllability of \systemname\ emulate link optimizations to remove (\ie, ``fill") null subcarriers.
%  \begin{minipage}[t]{0.24\textwidth}
%      \centering
%      \includegraphics[width=\linewidth]{pix/Eval_array_control.pdf}
%      \caption{CDF of controllability of the 36-element \systemname\ array across 30 links (pairs of Tx and Rx location). }
%      \label{fig:Eval_array_control}
%   \end{minipage}\hfill

\begin{figure*}
   \begin{minipage}[t]{0.32\textwidth}
     \centering
     \includegraphics[width=0.9\linewidth]{pix/Eval_chan_decompose.pdf}
     \caption{Predicted and measured phase difference for constructive superposition.}
     \label{fig:Eval_chan_decompose}
   \end{minipage}\hfill
%   
   \begin{minipage}[t]{0.32\textwidth}
     \centering
     \includegraphics[width=0.9\linewidth]{pix/Eval_Gap2OPT.pdf}
     \caption{Percent improvement of \systemname\ compared with exhaustive search.}
     \label{fig:Eval_Gap2OPT}
   \end{minipage}\hfill
%   
    \begin{minipage}[t]{0.32\textwidth}
     \centering
     \includegraphics[width=0.9\linewidth]{pix/Eval_SISO_MRD.pdf}
     \caption{Channel capacity achieved by MRD \cite{mrd-mobicom05}, \systemname, and MRD+\systemname.}
     \label{fig:Eval_SISO_shan}
   \end{minipage}
%   \vspace{-5pt}
\end{figure*}

\paragraph{\systemname\ element controllability.}\label{s:eval:micro:ele_control}
We define the difference between the maximum and the minimum \change{signal strength} that one \systemname\ element can induce at a particular subcarrier as the \textit{element controllability}.
We vary the link distance from 2~m to \change{8~m}, and measure the controllability of each individual \systemname\ element, \change{over three different links, for each link length.} Due to frequency\hyp{}selective fading, the environmental channel differs across subcarriers, which leads to differences in controllability. To investigate this effect, we \change{separate subcarriers into \emph{strong} ($[-53, +\infty]$~dBm), \emph{middle} ($[-65, -53]$~dBm), and \emph{weak} ($[-\infty, -65$~dBm) strength ranges and test the controllability of each subcarrier.  Figure~\ref{fig:Eval_control} shows the distribution of controllability across different \systemname{} elements, with one curve per physical link and subcarrier strength combination.  We see that two-meter links have no strong subcarriers, while six meter and eight-meter links have the most weakest subcarriers.  We also see consistent controllability across link length after binning the data into the above subcarrier strength ranges. Overall the clear trend is for greater controllability for weak subcarriers than for medium and strong ones.} 



\change{Considering absolute controllability, elements at different locations achieve from \emph{ca.} 
0~dB to 7.5~dB apiece,
since their $40\degree$ directional antennas capture
differing amounts of RF signal from different transmitter locations.
As link distance increases, signal power received from each 
element decreases, resulting in generally higher controllability.}



\paragraph{\systemname\ array controllability.}\label{s:eval:micro:arr_control}
Given the modest amount of controllability a single \systemname{} element provides, we investigate 36 \systemname\ elements working together. \change{We configure the array to maximize link Shannon capacity. The SNR changes on each subcarrier of six representative links are shown on the y-axis of Figure~\ref{fig:Eval_scatter}.  This scatter plot plots the original signal strength of each subcarrier on the x-axis.  We see that \systemname{} improves the SNR for all subcarriers and generally the weaker the subcarrier, the larger the improvement.}

In a separate larger-scale experiment involving 30 links, we bin the subcarriers of each individual link into the top, middle, and lowest thirds by SNR. The controllability distribution is shown for each bin (respectively, \emph{strong}, \emph{medium}, and \emph{weak} in Figure~\ref{fig:Eval_array_control}).
From the figure, we can see that \systemname{} provides up to 42~dB controllability. Median controllability for the strongest, medium, and weakest bins is about 10.4~dB, 11.8~dB, and 27.3~dB, respectively. In summary, multiple elements provide substantial controllability, especially when transceivers experience poor channel conditions.
%\begin{table}[t]
 % \centering
 % \begin{tabular}{M{1.6cm} M{1.32cm} M{1.3cm} M{1.2cm} M{1.0cm}}
 %   \toprule
 %   CSI reading & Phase computation & Element control & All\\
 %   
 %    4.9 $\pm$ 0.7 ms & 0.7 $\pm$ 0.04 ms & 0.085 $\pm$ 0.015 ms & 5.7 $\pm$ 0.7 ms \\
 %   \bottomrule
 % \end{tabular}
 % \caption{Time cost for controlling \systemname\ element.}
 % \label{tab:table1}
%\end{table}




% \begin{figure}[h]
%   \begin{center}
%       \includegraphics[width=0.8\linewidth]{pix/Eval_SISO_MRD.pdf}
%       \caption{CDF of channel capacity achieved by the environmental channel, MRD, \systemname, and MRD+\systemname.}
%       \label{fig:Eval_SISO_shan}
%   \end{center}
%   \vspace{-15pt}
% \end{figure} 

% \textcolor{blue}{Longfei: please briefly explain the experiment setups, how many experiment you run here. which channel you use? what does 31.2\% channel mean?}
\paragraph{Accuracy of channel decomposition.}\label{s:eval:micro:chan_decompose}
We next evaluate the accuracy of the channel decomposition algorithm. In these experiments, we randomly select a 2.4~GHz Wi-Fi channel and estimate the CSI of an individual \systemname\ element channel and the environmental channel using the channel decomposition algorithm presented in \S\ref{s:design:decomp}. With the decomposed channel, we compute the phase setting for this \systemname\ element that can maximize the reference SNR. At the same time, we apply different phases to this \systemname\ element to measure the difference between the computed phase setting and the real phase setting that maximizes SNR. Since the accuracy of the computed phase setting is only determined by the accuracy of channel decomposition algorithm, we can use the deviation between the computed and real phase setting as a metric to measure channel decomposition accuracy.

We repeat the phase decomposition test 2,000 times with different \systemname\ elements and different transmitter/receiver locations and plot the absolute phase difference between the computed and real phase settings in Figure~\ref{fig:Eval_chan_decompose}. 
% In the figure, The CDF shows . 
We can see that 85.4\% of the \systemname\ elements can be configured within an error of one phase shift step ($\pm 1/8 \pi$) and 99.4\% of the \systemname\ elements can be configured within an error of two phase shift steps ($\pm 1/4 \pi$). Based on our experience, we attribute most of the error to the small phase oscillation of phase shifters.

\paragraph{\systemname\ control algorithm--optimal gap.}
\label{s:eval:micro:gap_to_opt} 
We evaluate the gap between the \systemname\ control algorithm and optimal exhaustive search. We conduct extensive trace-based simulations on both SISO OFDM links and 4x4 MIMO OFDM links. We collect 5,000 traces for both cases, one trace for each link. Each trace includes the environmental channel and each \systemname\ element's channel. 
In order to make the comparison feasible within reasonable time, we consider a subset of the search space: five \systemname\ elements, each having eight phases. Consequently, exhaustive search can find the answer in $8^5 = 32,768$ search combinations for each trace. We compute the Shannon capacity of the result of both the \systemname\ control algorithm and exhaustive search. Additionally, we use percent Shannon capacity increase $\frac{C(\text{\systemname}) - C(\text{Env})}{C(\text{Opt}) - C(\text{Env})}$ as a metric to evaluate how close the \systemname\ control algorithm approaches the optimal. 

We observe in Figure~\ref{fig:Eval_Gap2OPT} that the \systemname\ control algorithm provides a close approximation of the optimal. For SISO OFDM, \systemname\ finds the exact optimal in 80.76\% of the cases. For 4x4 MIMO OFDM, \systemname\ finds the exact optimal in 61.6\% of the cases. On average, \systemname\ can achieve 99.23\% and 96.89\% capacity increase compared to the optimal solution for SISO and 4x4 MIMO cases, respectively.

% \subsubsection{Control delay}
% We also evaluate the control delay of \systemname\ system. To program the \systemname\ element to shift a proper amount of phase, we need to 1): read CSI from the receiver; 2): compute the phase that can achieve constructive combination; 3): set the phase shifter of the \systemname\ element accordingly. 
% We term these three control steps an entire control process.
% We then repeat this entire control process 5,000 times and compute the average delay and standard deviation of each control step. 
% As shown in Table~\ref{t:Ctl_Delay}, reading the CSI accounts for the majority of the \systemname\ control delay since the CSI is delivered through Ethernet in our system. 
% The phase calculation and element control only takes around 1/7 and 1/50 of the CSI reading time.
% The overall average delay of the entire control process is within 5.7~$ms$, during which the channel is still relatively stable.

\paragraph{Element density.}
\change{We evaluate the impact of \systemname{} element density in the array. Our 36-element array is deployed on a $2 \times 1.8$~m wall. We build a 9-element array by selecting nine adjacent elements from a $0.7 \times 0.5$~m wall area and measure the controllability of each such array. We then build another 9-element array by randomly selecting nine elements from all 36 elements. We repeat this random selection process 1,000 times. The controllability (averaged over subcarriers) achieved using nine adjacent and nine randomly selected elements (averaged over 1,000 experiments), is 2.57~dB and 2.50~dB, respectively.  We see that the density of the \systemname\ elements does not significantly affect achieved controllability.}

==> intro_attic.tex <==
In short video, the location of the user swipe determines the playing order of video chunks, 
which is fundamentally different from any other video streaming applications.
If the user swipe happens at the end of one video, \ie, the case one in Figure~\ref{fig:intro_view_seq},
all of its chunks will be played sequentially, just as in any other traditional video streaming applications. 
But if the user swipes during the playback of one video, \ie, the case two in Figure~\ref{fig:intro_view_seq},
the video player immediately terminates the playing of the current video,
skips the playing of chunks after the swipe, 
and switches to the beginning of the next video.  

The randomness bring by the user swipe makes the chunk download scheduling of short video very challenging.
Ideally, if we know the exact location of the user swipes, 
we can determine the optimal chunk downloading sequence based on two rules:
the chunk played first should be downloaded first 
and we should skip the downloading of the chunks that are not played due to swipes,
just as shown in Figure~\ref{fig:intro_view_seq}.
However, in practice, we must determine the downloading sequence before the user swipe,
since the downloading of chunks must finish before its playing, 
\eg, as shown in case two of Figure~\ref{fig:intro_view_seq}, 
the downloading of the first chunk in the second video must be finished 
before the actual swipe to prevent rebuffering from happening.
Accurately predicting the location of the user swipes is a possible solution for determining the downloading sequence,
which, however, has proven to be challenging for interactive video apps.

To understand how state-of-the-art commercial apps determines the downloading sequence,
we conduct, to the best of our knowledge, the first of its kind measurement study on 
the most popular commercial short video app---TikTok.
We observe that TikTok divides one video into two chunks and apply fixed rules
to determine the downloading sequence:
always prioritizing the downloading of the first chunk 
and delaying the downloading of the second chunk of a video until the first chunk of the video is being played. 
Such a fixed rule cannot handle the diverse swipe patterns across videos and users, 
\eg, in the case two of Figure~\ref{fig:intro_view_seq}, 
we should prioritize the downloading of the second chunk of first video 
if the user continues watching the first video instead of swiping after watching the first chunk.


%R\rn{one of your big contributions is the study of tiktok (which I think is first of its kind). emphasize that you did the first study (to our knowledge) to uncover how state-of-the-art commerical apps deal with the challenges of short videos (that prior ABR strategies don't handle). then say whey they are bad...}
%R

%Traditionally, video players use adaptive bitrate (ABR) algorithms to maximize user's QoE. 
%These algorithms run on the client side. 
%For each video, the algorithm initializes its own states from the video's manifest file 
%and periodically determines the bitrate of next video chunk that the player is going to fetch from the content server. 
%However, the traditional ABR algorithms does not work for short video streaming application for three reasons. 
%(1) Existing ABR algorithms does not have a mechanism to buffer video chunks across multiple videos, 
%which will incur significant rebuffering time when user swipe to get the next video. 
%(2) Traditional ABR algorithms will be stuck in the startup phase when working for short video streaming, 
%since they have to re-initialize states from the manifest file for every new video. 
%(3) In addition, traditional ABR algorithms buffer video chunks sequentially. 
%The buffered video chunks will be discarded once the user swipe and switch to the next video, 
%which causes a waste of the network bandwidth and further decreases users' QoE. 
%\rn{hmmm I'm not quite sure I get the key issues. 
%\#1 seems implementation-y, e.g., the prior works can just view all the short videos as one continuous one. the issue seems to be much more around swipes! this needs to be emphasized.}


%The main task of the short video app is to schedule the order of the video chunks that the app downloads in the future.
%The app then obtains the optimal video bitrate of each chunk by 
%feeding the downloading sequence to the existing video streaming ABR algorithms like MPC~\cite{yin2015control}.
%Generally, to maximize the QoE, the order of the downloading chunks 
%must follow the order of the video chunks that the user watches.
%Therefore, scheduling the downloading sequence is straightforward for traditional 
%long video streaming like YouTube or Netflix, where the viewing sequence of a long video is fixed.
%
%The above heuristic cannot apply to interactive short video streaming, 
%since there exists multiple possible viewing sequences due to the randomness in the timing of the user swipes.
%For example, as shown in Figure~\ref{fig:download_budget},
%when watching the first video with three chunks, the user may swipe at the end of all three chunks,
%resulting in three possible viewing sequence. 

%\rn{one of your big contributions is the study of tiktok (which I think is first of its kind). emphasize that you did the first study (to our knowledge) to uncover how state-of-the-art commerical apps deal with the challenges of short videos (that prior ABR strategies don't handle). then say whey they are bad...}
%
%\rn{in this transition, I think a nifty flow could be around how having perfect swipe predictions would eliminate the problem (and make prior works sufficient). 
%but modeling user behavior accurately has proven challenging for interactive video apps. 
%instead, the core insight we have is that we don't need perfect modeling! we do a study of X users with real short video app 
%to understand that while user swipes are hard to model, when aggregated on a given video, the distribution is quite stable and sufficient to make robust decisions.} 
%


\textcolor{red}{To be finished. Not very clear in my mind now.}
Our core insight is that 
1, user swipe pattern inside a video is stable from our user study
2, we don't need the perfect user swipe pattern. 
we can determine the video downloading sequence even only using chunk level user swipe pattern
To determine the downloading with 

\textcolor{red}{To be finished}
In this paper, we present the design and implementation of \systemname, 
a video bitrate adaptation system for short video streaming. 
To enable seamless transition between short videos, 
\systemname\ adopts an out-of-order prebuffering mechanism, 
which allows prebuffering for future videos before the prebuffering for current playing video finishes. 
With a deep analysis of the traditional video streaming algorithms and existing short video applications, 
\systemname's ABR algorithm optimizes the expected quality of experience during the short video streaming. 
Specifically, \systemname\ models and derives the  transition probability between consecutive videos caused by user's swipe. 
With the transition probability, \systemname's ABR algorithm applies a model predictive control (MPC) based algorithm to maximizes the quality of experience. 

\systemname{} is a new video streaming algorithm that aims to deliver high QoE despite the unpredictability in user swipe patterns (and thus video/chunk viewing sequences). Importantly, \systemname{} is directly deployable in the client-side components of existing short streaming applications, and requires no changes to videos, network protocols, or servers. 


\textcolor{red}{To be finished}
We implemented our system 
Extensive experimental results show that 

% \begin{itemize}
%     \item 1. User generate content with AR effect
%     \item 2. Social apps following the celebrities
%     \item 3. Immersive experience, the user can proceed to next video with swipe
% \end{itemize}




==> tiktok_attic.tex <==
%The ABR algorithm makes its decision according to the network capacity, buffer status and user swipes.
%The app translates the results of ABR into HTTPS requests to fetch short videos from the CDN.
%We could also observe the impact of ABR algorithm on the screen, such as the video quality and rebuffering events.
%To conduct a controlled experiment to understand the ABR algorithm of TikTok, 
%we use Mahimahi~\cite{netravali2015mahimahi} to control the network throughput from TikTok app to its CDN server
%and implement an automatic swipe tool to input a pre-defined swipe pattern to the app. 
%We also develop a screen analysis tool to record the playing progress of each video and 
%log the starting timestamps and duration of every detected rebuffering events.

%\paragraph{Challenge.}
%The TikTok is installed on mobile devices as a closed-source app.
%Without accessing the source code, we cannot know the internal status of TikTok, 
%such as the buffer status
%%number of videos and the number of chucks of each video that has been buffered,
%and the content of HTTPS requests that have been sent.
%Sniffing the network to extract the content of every HTTPS request does not work 
%since all the HTTPS traffic are end\hyp{}to\hyp{}end encrypted.


%The commercial short video streaming services like TikTok are implemented as smartphone applications 
%to provide the immersive experience for users. 
%It is not feasible to use web browser based traffic analysis tools to understand the ABR strategy for APP-based short video services. 
%To accomplish this challenge, we develop a tool chain to understand the ABR decisions made by the smartphone applications on Android. 
%The tool includes three major components. 
%One is a proxy that serves as the man in the middle to record downloading requests of all the video and manifest files. 
%The second component is a screen analysis tool to record the progress of the video and rebuffering events. 
%The third component is an automatic swipe tool to view the short video at an arbitrary pace. 
%All the three components are deployed on the same computer to get synchronized timestamps of events.

%\paragraph{Decrypting the HTTPS request.}
%\textcolor{red}{TODO: explain the process}
%As shown in the Figure~\ref{fig:tool}, 
%the proxy is deployed in the same local area network with the smartphone running the short video application. 
%We rooted the Android phone and patched the Android system to send all request from the short video application through the proxy. 
%To handle the Secure Sockets Layer in HTTPS, we patched the certificate of the proxy into the rooted Android system and 
%disabled the SSL pining of the short video application with Android Debug Bridge and a reverse engineering tool~\cite{frida}. 
%This allows us to decode meaningful information from the HTTPS requests on the proxy. 
%The proxy forwards the request to the CDN server and the response  back to the short video application. 
%The proxy logs the requests and response information including available bit-rates in the manifest, 
%video download bit-rates, video downloading time etc. 
%In addition, we run the proxy within the Mahimahi~\cite{netravali2015mahimahi} shell so that 
%we can control the network throughput from TikTok application to its CDN server with an arbitrary network trace.

%The screen analysis tool records all the rebuffering events and video playing progress with vision based algorithms. 
%To enable the screen analysis tool, we mirror the screen of the smartphone to the Linux desktop via USB cable. 
%The screen analysis tool running in the desktop then can directly use a vision-based algorithm to compute when the rebuffering starts.

%The automatic swipe tool can swipe to the next short video in an arbitrary pace. 
%The swipe changes the buffer length by skipping the unplayed content of the current video. 
%By varying the pace of swipe, the tool can explore and record the ABR decisions of short video application under different buffering lengths. 
%In addition, it will record the timestamps of the swipe for the purpose of analysis and replay.

%\paragraph{Inferring the buffer status.}
%\textcolor{red}{TODO: Explain the HTTP request content and maybe add a figure to demonstrate how to extract the buffer status.}

%\subsubsection{Measurement Result.} 
%\label{ss:measurement-result}
%With the measurement tool shown in Figure~\ref{fig:tool}, we can perform in-depth analysis through recorded logs. We present measurement result to answer three questions: (1) What is TikTok's video format?
%(2) How TikTok decides the download order?
%(3) How TikTok decides the download bitrate?


%\subsubsection{Basic Design Choices}


%\paragraph{Video format.} 
%Surprisingly, we observe from the \textcolor{red}{manifest file?} that 
%TikTok uses MP4 as its video format rather than DASH or HLS,
%which probably saves the cost of adapting the video format between Android (DASH) and IOS (HLS) devices. 



%TikTok, however, divides the video into no more than two chunks, 
%since the short videos are generally short, \ie, \textcolor{red}{less than 60 seconds}.



%since because 
%Such a chunking strategy allows TikTok to minimize the chances of rebuffering after user swiping 
%by pre\hyp{}buffering only the first chunk of the following few videos.



%Besides the choice of maximum two chunks per video, 
%%another interesting design choice of TikTok is that it splits the first and second parts with the number of bytes rather than the time in the playback. 
%another interesting design choice of TikTok is that it splits the video according to the video size instead of video length in playback time. 
%Our hypothesis is that it allows TikTok to pre\hyp{}buffer the first part of a video 
%with a fixed download time expectation without considering the bitrate variation on different videos. 
%However, this mechanism prevents TikTok from switching the bitrate between the first-part and second-part video, 
%which could lead to possible premature bitrate binding, which will discussed in \S\ref{ss:tiktok-result-analysis}.

%Each video is encoded with several video control knobs, including the frame rate, 
%the resolution, and the quantization parameters. 
%We denote a specific combination of video control knobs as a \textit{nominal bitrate} for the video. 
%Different videos encoded with the same nominal bitrate 
%may have different actual bitrates (in bytes) due to the differences in the video content. 

%If the size of a video is more than 1,000 KB, the TikTok's content server will split it into two parts: 
%the first part includes the first 1,000 KB of data and the second part has the rest of the video. 
%During the video play, the user is able to watch first a few seconds of video even if only the first part is downloaded. 
%With this mechanism, TikTok's ABR algorithm could reorder the download sequence of the second part of a early video in the watch sequence 
%and the first part of a later video. This allows the ABR algorithm hedges against the uncertainty of users' swipe. 
%We observe from Figure~\ref{fig:playback-demo} that TikTok requests exactly the same bitrate for two chunks inside one video. 
%We also confirmed such an observation by examining the bitrate of the two chunks inside 1200 short videos.
%Such a mechanism significantly limits the TikTok's capability of adjusting the video bitrate 
%according to the variations in network capacity.
%As a comparison, DASH allows video bitrate adaptation at the granularity of chunk level.


%Each video is encoded with several video control knobs, including the frame rate, 
%the resolution, and the quantization parameters. 
%We denote a specific combination of video control knobs as a \textit{nominal bitrate} for the video. 
%Different videos encoded with the same nominal bitrate 
%may have different actual bitrates (in bytes) due to the differences in the video content. 

%We have two observations of the TikTok bitrate.
%First, the first and the second chunk of the same video have the same nominal bitrate,
%which significantly limits the ABR's capability of adjusting the video bitrate according to the variations in network capacity.
%As a comparison, DASH allows video bitrate adaptation at the granularity of chunk level.

%Second, videos streamed by the CDN have varying number of nominal bitrate choices,
%\textcolor{red}{TODO: add data and explain}


%The TikTok server and client exchanges the information 
%of the next 10 videos that the server will stream to the client 
%via one \textit{manifest file}. 
%Inside this manifest file, the server includes the available bitrate, the number of chunks (one or two) 
%and the location (IP of the corresponding CDN) of all 10 videos. 


%\paragraph{Impact of buffer status.}
%To investigate the impact of buffer status, \ie, the number of buffered first chunk, 
%on TikTok's buffering strategy,
%we conduct a controlled experiment by setting the network capacity to 10~Mbit/s using Mahimahi.
%We note that 10~Mbit/s is a high capacity that 
%allows the TikTok to download the first chunk of a video within one seconds.
%%\textcolor{red}{seems not high enough}.
%During this experiment, TikTok downloads 80 videos. 
%We measure the number of buffered first chunks when TikTok starts downloading all the 80 videos and 
%plot the results
%in Figure~\ref{fig:10mbps}.
%%Each time TikTok decides to download the first chunk of a new video, we log the buffer status 
%%We plot the buffer status, \ie, the number of downloaded first chunks inside the buffer, 
%%at the time point when TikTok makes a decision to download the first chunk of each video, 
%%in Figure~\ref{fig:10mbps}.
%We see that TikTok's chunk downloading is driven by the buffer status. 
%In the beginning of downloading one video group,
%the downloading is driven by the fact that the number of buffered first chunks is smaller than five.
%In the steady state, the downloading is driven by the event that the number of buffered videos decreases to four.
%
%Within each group, TikTok aggressively downloads new videos in the beginning until accumulating five first chunks.
%In the steady state, TikTok starts downloading a new first chunk when the number of buffered videos decreases to four.
%%To better demonstrate the time correlation between the first chunk downloading and the decreasing of buffered video in steady state,
%%we plot the variations of buffered videos and the first chunk downloading event in 
%%Figure~\ref{fig:buffer_download_event}, 
%%from which we could see that the timestamps of the video downloading coincides with the buffer status change. 
%At last, TikTok does not start downloading the videos of next video groups
%unless the number of buffered first chunks decreases to one. 
%\begin{figure}[htb]
%    \centering
%    \includegraphics[width=\linewidth]{pix/Buffer_download_event.pdf}
%    \caption{
%    The number of buffered first chunk varies with time, which triggers the video downloading.
%    \textcolor{red}{I need to update this figure to clearly emphasize our pionts.}}
%    \label{fig:buffer_download_event}
%\end{figure}

%\noindent
%\textit{Takeaway:}
%TikTok adopts a buffer driven video downloading algorithm.
%Specifically, TikTok tries to guarantee that
%%the goal of TikTok's video buffering strategy is to try its best effort to guarantee that,
%no matter when the playing video switches to the next one (due to user swipe or video playing finishes),
%there is at least one and at most five first chunks of different videos already downloaded and stored inside the buffer.
%
%\begin{figure}[htb]
%    \centering
%    \includegraphics[width=\linewidth]{pix/Bitrate.pdf}
%    \caption{The video bitrate TikTok selects for downloading 80 videos from network with 10~Mbit/s and 3~Mbit/s.
%    The bitrate index 1, 2, 3, and 4 represents the bitrate of 480p, 520p high, 520p low and 720p, respectively.}
%    \label{fig:bitrate}
%\end{figure}
%


%\noindent
%\textit{Takeaway:}
%TikTok prioritizes video buffering over video bitrate. 
%The primary goal of TikTok is to accumulate and 
%then maintain enough pre-buffered video chunks inside the buffer,
%even at the cost of decreased video quality. 

%no first chunk downloading after it finishes downloading one group of video, until there are only two buffer

%To illustrate TikTok's video downloading strategy, 
%we plot a time-series of video chunk downloading event of the TikTok in Figure~\ref{fig:playback-demo},
%from which we have two observations.
%\begin{figure}[htb]
%    \centering
%    \includegraphics[width=0.6\linewidth]{pix/time_diff.pdf}
%    \caption{
%    The time difference between the start of playing the first chunk of one video 
%    and the start of downloading its second chunk.}
%    \label{fig:time_diff}
%\end{figure}


%\begin{figure}[htb]
%    \begin{minipage}[htb]{0.4\linewidth}
%        \centering
%        \includegraphics[width=\textwidth]{pix/time_diff.pdf}
%        \caption{The time difference between the playing of the first chunk of a video
%    and the downloading of its second chunk.}
%        \label{fig:time_diff}
%    \end{minipage}
%    \hfill
%    \begin{minipage}[htb]{0.58\linewidth}
%        \centering
%        \includegraphics[width=\textwidth]{pix/download_2nd_chunk.pdf}
%        \caption{The playing of a new video could trigger the downloading of two chunks: 
%        the second chuck of the currently playing video and 
%        the first chunk of a new video. }
%        \label{fig:download_2nd_chunk}
%    \end{minipage}
%\end{figure}
%
%\paragraph{Automatically downloading the second chunk.}
%%TikTok spends a lot of effort on maintaining enough number of downloaded first chunk of video. 
%%We have introduced how TikTok buffer the first chunk of videos.
%%TikTok adopts a relatively simple mechanism to schedule the downloading of the second chunk.
%TikTok automatically triggers the downloading of the second chunk of a video
%when the TikTok begins to play that video, just as shown in Figure~\ref{fig:playback-demo}.
%To further verify that, we plot the CDF of the time difference between 
%the start of playing the first chunk of 1200 videos 
%and the start of downloading their second chunks
%in Figure~\ref{fig:time_diff}.
%We see that the time difference is smaller than 0.61 second for 95\% of the videos,
%which demonstrates the connection between the video playing and second chunk downloading.
%
%The playing of a new video not only triggers the downloading of its second chunk, 
%but also consumes one first chunk in the buffer,
%which triggers TikTok in steady state to download a new first chunk to maintain five videos available inside the buffer.
%%As a result, the playing of a new video could simultaneously trigger the downloading of two possible chucks:
%%the second chunk of the playing video and the first chunk of a new video.
%We observe that TikTok prioritizes the downloading of the second chunk of the playing video 
%over the downloading of a new first chunk,
%just as shown in Figure~\ref{fig:download_2nd_chunk}.

%
%First, the TikTok only pre\hyp{}buffers the first chunk of each video 
%and starts downloading the second chunk when and only when the first chunk is being played and watched by the user.
%By doing so, the TikTok significantly simplifies the problem.
%Specifically, TikTok only needs to determine the timing and video quality of the first chunk,
%while the configuration of downloading the second chunk is determined automatically,
%\textit{i.e.,} the quality is the same as the first chunk and 
%the downloading timing is the same as the video playing time of the first chunk. 
%Such a strategy, however, causes excessive video downloading (the TikTok cannot cancel an ongoing video chunk downloading),
%especially when the user quickly swipes to the next video,
%resulting in huge waste of network capacity.
%\textcolor{red}{We need some data to back it up here.}

%TikTok splits a video into two parts and download them separately. 
%It is critical to determine when TikTok app start to download the two video parts for the sequence of video in the playback. 
%Second, to determine the downloading timing and order of the first video chunk,
%the TikTok implements an algorithm that consists of three phases:
%%The first part of the video is downloaded in the same order as the playing sequence. 
%%The time to issue the download request for the first video parts depend on the states of the playback. 
%%Specifically, TikTok schedule the download of first video parts by the group of ten videos. 
%%Each scheduling group includes three periods: 
%ramp-up period, buffering maintaining period, idle period. 
%(1) \textbf{Ramp-up period} corresponds to the red zones in Figure~\ref{fig:playback-demo}. 
%In this period, TikTok sends download request consecutively to build up the buffer until there are five future first-part videos in the buffer. 
%(2) After that, the ABR algorithm enters the \textbf{Buffering maintaining period}, which corresponds to the green zones in Figure~\ref{fig:playback-demo}. 
%In this period, TikTok maintains the total number of first-part videos to be five. 
%It downloads a new first-part video once the user switches to the next video in the playing sequence. 
%Buffering maintaining period ends when the video index modulo ten equals to zero. 
%(3) The ABR algorithm then enters the \textbf{Idle period}. 
%In this period, TikTok will not download the first-part video. 
%The Idle period ends when the number of first-part videos drops to two 
%and then the algorithm enters the ramp-up period of a new scheduling cycle. 


%The download time for the second video part is relatively simple. 
%As shown in Figure~\ref{fig:playback-demo}, TikTok downloads the second part of the video (the hatched progress bar in the figure) 
%when the video starts to play (the dashed line segment in the figure).
%TikTok inserts the download request for the second-part video into the download sequence of the first-part videos but will not discard the on-going download requests. 

%\paragraph{Summary of TikTok.}
%We summarize TikTok's video downloading and bitrate adaptation algorithm as follows:
%
%\begin{itemize}
%\item \textit{Periodical buffer accumulation and draining.}
%TikTok first aggressively download first chunks to fill the buffer 
%and maintain constant buffer level until all the first chunks of 10 videos in the same group are downloaded.
%After that, TikTok drains the buffer till only one first chunk left.
%
%
%\item \textit{Buffer driven first chunk downloading.}
%TikTok schedules the downloading of the first chunk according to the current buffer status. 
%
%
%\item \textit{Automatic second chunk downloading.}
%TikTok automatically triggers the downloading of the second chunk after the playing of this video.
%
%\item \textit{Throughput based bitrate adaptation.} 
%TikTok selects the bitrate of the video purely based on the available network throughput.
%\end{itemize}

%\begin{figure}
%    \centering
%    %\includegraphics[width=\linewidth]{pix/video_download.pdf}
%    \begin{subfigure}[t]{0.58\linewidth}
%      \centering
%      \includegraphics[width=\linewidth]{pix/RateAdaptation.pdf} % changed
%      \caption{The time lag between chunks.}
%      \label{fig:rate_time_diff}
%  \end{subfigure}\hfill
%  \begin{subfigure}[t]{0.41\linewidth}
%      \centering
%      \includegraphics[width=\linewidth]{pix/TimeLag.pdf} % changed
%      \caption{CDF of time lags.}
%      \label{fig:rate_cdf}
%  \end{subfigure}\hfill
%    \caption{
%    The time lag between the downloading of the first and second chunk of the same video.
%    Since TikTok buffers five first chunks so the first chunk of the $n^{\mathrm{th}}$ video 
%    may already been downloaded when the user is watching $n-5^{\mathrm{th}}$ video~\textbf{(a)}.
%    The CDF of the time lag between two chunks for 1,200 videos is given in~\textbf{(b)}. }
%    \label{fig:rate_adaptation}
%\end{figure}

%\begin{figure*}
% Number of virtual camera real testbed
%  \begin{subfigure}[t]{0.33\linewidth}
%      \centering
%      \includegraphics[width=\linewidth]{pix/all_distribution.pdf} %% changed
%      \caption{The distribution of average viewing percentage %across all short video views.}
%      \label{fig:swipe-total}
%  \end{subfigure}\hfill
%    \begin{subfigure}[t]{0.33\linewidth}
%      \centering
%      \includegraphics[width=\linewidth]{pix/swipe_time.pdf} % %changed
%      \caption{The distribution of average viewing time for %different users.}
%      \label{fig:swipe-videotime}
%  \end{subfigure}\hfill
%    \begin{subfigure}[t]{0.33\linewidth}
%      \centering
%%      \includegraphics[width=\linewidth]{pix/kl.pdf} % changed
 %%     \caption{KL divergence of swipe distribution over the same v%ideo between two datasets.}
%      \label{fig:swipe-kl}
%  \end{subfigure}
%   \caption{User swipe statistics for both mobile web dataset and %Mturk dataset.}
%   \label{fig:user-swipe}
%\end{figure*}

%Therefore, there is only one buffered first chunk when it starts downloading the first video of the next video group.
%We illustrate the detailed buffer draining process in Figure~\ref{fig:group_trans}.

%\paragraph{Coarse-grain video bitrate adaptation}
%TikTok adjusts its bitrate at the granularity of video level instead of chunk level.
%We note that there exists a large time lag between the downloading of the first and second chunk of one video.
%Specifically, since TikTok buffers five first chunks so the first chunk of the $n$\hyp{}$th$ video 
%may already been downloaded when the user is watching $(n-5)$\hyp{}$th$ video, just as shown in Figure~\ref{fig:rate_time_diff}.
%We plot the CDF of the time lag between two chunks for 1200 videos in Figure~\ref{fig:rate_cdf},
%from which we could see that the median time lag is 25.3 seconds.
%
%TikTok selects the bitrate according to the instantaneous network throughput at the moment of downloading the first chunk.
%Such a throughput, however, may change dramatically at tens of seconds later when TikTok downloads the second chunk. 
%The mismatch between the selected video bitrate and the current network throughput could significantly enlarge the downloading time of the second video chunk
%and delay the following scheduled downloading of the first chunks of other videos.
%
%
%- Bullet for the summary of
%tiktok algorithm
%- Despite targeting short video streaming environment, we find that TikTok often leads to suboptimal performance in realistic settings: X-Y\% gap from optimal, with substantial rebuffering (X-Y seconds) in low-bandwidth settings.
%- Digging deeper, the reason is largely due to TikTok's generic approach to dealing with the uncertainty of potential swipes, i.e., they don't adapt their algorithm to different videos/users. Instead, they follow a very generic approach that is often too cautious or aggressive. This manifests in two particular ways with the goal of minimizing issues with fast swipes:
%* buffer ordering (always get next 5 first chunks)
%* byte-based chunking (chunks are 1MB to have certainty in sizes/download times, rather than chunking based on time which can be variable size due to encoding and video content) --> this ties them into a bitrate for the second part of that chunk when it is needed (and the network could be totally different then) [by design, the algorithm is downloading first parts really early, so it is likely that the network will be different]
%
%- to understand why such fixed patterns are bad, in the next section we examine swipe patterns across real users and videos.
%
%[big takeaway: tiktok doesn't seem to consider swipe info or predictions, and instead deals with the uncertainty of potential swipes in a cautious/generic way.]


%\begin{figure}[t]
%    \centering
%    \includegraphics[width=\linewidth]{pix/RateAdaptation.pdf}
%    \caption{The impact of network throughput and buffer level on the encoded video bitrate.\textcolor{red}{update}}
%    \label{fig:group_trans}
%\end{figure}


%While there is no significant clues that show the bitrate is correlated to the buffer level. 
%It is likely that TikTok's algorithm makes the bitrate decision based on the throughput estimation. 

% \subsection{Result Analysis.} 
% \label{ss:tiktok-result-analysis}

%Based on our interpretation of the measurements,  
%we list the following two limitations of TikTok's video buffering and bitrate adaptation algorithm.
%the measument above, we list three problems of TikTok's ABR algorithm and then discuss the possible improvement that could be made. 

%\begin{figure}[htb]
%    \centering
%    \includegraphics[width=\linewidth]{pix/GroupTransition.pdf}
%    \caption{TikTok drains its buffer after it finishes downloading the current video group.} 
%    \label{fig:group_trans}
%\end{figure}
%
%\paragraph{Periodic buffer draining and accumulating.} 
%{\color{red}To change to lack prediction}
%%Just as shown in Figure~\ref{fig:buffer_download},
%TikTok maintains five downloaded first chunks in steady state 
%and then drains buffer after it finishes downloading all 10 videos inside the current video group.
%We use an example in Figure~\ref{fig:group_trans} to illustrate such a process in detail.
%In this example, TikTok finishes downloading the first chunks of all 10 videos when the user is watching the 4\hyp{}$th$ video.
%After that, TikTok stops downloading but continues video playing that drains the buffer.
%TikTok starts downloading the video of next group when there is only one first chunk left in the buffer.
%The buffer draining process also explains the sudden decrease in number of buffered videos 
%at the boundary of video groups in Figure~\ref{fig:buffer_download}.
%After starting fetching the videos from a new group, 
%TikTok downloads multiple video at maximum speed to accumulate the buffer as soon as possible, 
%causing a burst of video chunk downloading, just as shown in Figure~\ref{fig:group_trans}.
%
%Such a periodic buffer draining and accumulating scheme may easily result in rebuffering event.
%For example, if TikTok cannot finish downloading the first chunk of the 10\hyp{}$th$ video when the user is watching the 8\hyp{}$th$ and 9\hyp{}$th$ videos,
%the number of buffered video reduces to zero and rebuffering event happens, just as shown in Figure~\ref{fig:group_trans}.
%Such a case happens if the network throughput is low and hence the downloading takes long time 
%or the user quickly skips the 8\hyp{}$th$ and 9\hyp{}$th$ video with two consecutive swipes 
%and hence the time budget for downloading 10\hyp{}$th$ video becomes small.


%In a mobile network, the network throughput could change dramatically after 25.3 seconds.
%Therefore, there exists an obvious mismatch between the video bitrate selected 
%so the bitrate selection happens in tens of seconds cannot work ago may not 

%\paragraph{Lack of swipe prediction.} 
%As shown in \S\ref{ss:measurement-result}, 
%TikTok decides the download sequence and timing based on a set of fixed rules without considering the users' swipe patterns: 
%TikTok always inserts the second-part video download into the download sequence when the video starts to play. 
%When the user swipes quickly, this mechanism could lead to rebuffer at the first-part of later videos. 
%If the user did not swipe on the video, this mechanism could also lead to rebuffering at the second-part of current video when the network throughput is low. A possible improvement is to decide the downloading sequence based on the users' swipe distribution and prioritize the video downloading based on the watching probabilities. We believe TikTok already has swipe distributions but just apply it to ABR algorithms. We will show that even with the swipe distribution dataset that is fairly smaller than the scale of TikTok, we can still make a significant improvement in terms of quality of experience by reducing the rebuffering and the wasted video content (downloaded by not watched).
%
%\paragraph{Premature bitrate binding.} Another problem is that TikTok binds the bitrate of second-part video prematurely. TikTok cannot switch bitrate between the first-part and second-part videos since it splits two parts of video by number of bytes. That is to say the bitrate of a second-part video is decided based on the playback and network status when downloading the first-part video, which could be a dozens of seconds ago. This could introduce and exacerbate the rebuffering. For example, when the network is good, TikTok will choose a high bitrate to download the first-part video. When it starts to download the second-part video 30 seconds later, the network throughput drops. It will then causes a significant rebuffering before playing second-part video. The solution is to split different parts of video by time rather than bytes. But this requires a better ABR algorithm to handle the bitrate variation on different videos. 
%

% \begin{itemize}
%     \item \textbf{Lack of Prediction:} TikTok prematurely download the future first part. It downloads later videos' first parts rather than earlier videos' second parts. 
%     \item \textbf{Lack of Prediction:} TikTok did not download future videos' first parts far enough in the future. when the user has high probability to swipe to the next video. 
%     \item \textbf{Network Idling:} idling the network without 1.) increasing the video bit rate 2.) not downloading future 2nd parts 
%     \item \textbf{Premature Binding:} committing to the high video encoding bit rate for both 1st and 2nd parts at time of 1st part D/L. Why?  Our guess is TikTok wants to have a small and predictable time for 1st part D/L and then uses fixed 1000 KB for the size of the first part. This make it difficult for them to change the bitrate in the middle.
%     \item \textbf{Wasted bytes:} Download bytes the user never watches
% \end{itemize}
